Optimal Transport-based Alignment of Learned Character Representations for String Similarity

String similarity models are vital for record linkage, entity resolution, and search. In this work, we present STANCE --a learned model for computing the similarity of two strings. Our approach encodes the characters of each string, aligns the encodings using Sinkhorn Iteration (alignment is posed as an instance of optimal transport) and scores the alignment with a convolutional neural network. We evaluate STANCE's ability to detect whether two strings can refer to the same entity--a task we term alias detection. We construct five new alias detection datasets (and make them publicly available). We show that STANCE or one of its variants outperforms both state-of-the-art and classic, parameter-free similarity models on four of the five datasets. We also demonstrate STANCE's ability to improve downstream tasks by applying it to an instance of cross-document coreference and show that it leads to a 2.8 point improvement in B^3 F1 over the previous state-of-the-art approach.

==> neighbors.tex <==
%auto-ignore
\begin{figure*}
	\scriptsize
	\centering
	\begin{tabular}{c|c|c}
		 Sim-OT-CNN & Jaro-Winkler & LCS \\
		 \hline
		 Hicks, Bill & Hicks, Bill & Bill Hicks and His Sizzlin' Six\\
		 Bill Hicks and His Sizzlin' Six & Hocus Pocus & William Melvin Hicks\\
		 Bill Hilly Band, The & The Zombies & Bill Challis and His Orchestra\\
		 Bill Hilly Band, The & Jim Reevers & Bill Hickey\\
		 \hline
		 CPTP & Civilian Pilot Training Service & Civilian Pilot Training Service \\
		 Civilian Pilot Training Service  & civilian pilot training & Nutrition Education and Training Program \\
		 civilian pilot training & Castilian civil war & National Oceanic and Atmospheric Administration Climate and Societal Interactions Program \\
		 flight training program & civilian population & Department of Civil and Environmental Engineering, University of Illinois at Urbana-Champaign \\
	\end{tabular}
\caption{Predicted nearest neighbors for the queries "Bill Hicks" (top row) and "Civilian Pilot Training Program" (bottom row).}
\end{figure*}


==> noise-stacked.tex <==
%auto-ignore
\begin{figure}
  \begin{subfigure}[t]{0.75\textwidth}
    \centerline{\includegraphics[width=0.75\textwidth]{../figs/noise.png}}
    \caption{Similarity Matrix.}
    \label{fig:flex}
  \end{subfigure}
  \begin{subfigure}[t]{0.75\textwidth}
    \centerline{\includegraphics[width=0.75\textwidth]{../figs/noise-filter.png}}
    \caption{Noise Filtered}
    \label{fig:noise}
  \end{subfigure}
  \caption{\textbf{Noise Filtering:} OT effectively
    reduces noise in the similarity matrix even when many character
    n-grams are common to both mentions (Teen Bahuraaniyaan / Saath Saath Banayenge Ek Aashi).}
\end{figure}
